Shades of Finality and Layer 2 Scaling

Blockchains combine a distributed append-only log with a virtual machine that defines how log entries are interpreted. By viewing transactions as state transformation functions for the virtual machine, we separate the naming of a state from the computation of its value and reaching consensus on that value. This distinction allows us to separate the notion of transaction order finality from state value finality. Further consideration of how blockchain governance handles catastrophic failures such as zero day exploits leads us to the notion of checkpoint finality. Consensus on the transaction order determines the ground truth. Everything else -- computing the value of a state or handling catastrophic failures such as bugs / zero-day based attacks -- are just optimizations.

==> author-acm.tex <==
%\authorinfo{
%{\rm
%  Raymond Cheng$^{\dag}$,
%}\\
%{\small
%  $\dag$University of Washington
%}
%}

\fancyhf{} % Remove fancy page headers 
\fancyhead[C]{Anonymous submission \#103 to ACM CCS 2017}
\fancyfoot[C]{\thepage}

\setcopyright{none} % No copyright notice required for submissions
\acmConference[Anonymous Submission to ACM CCS 2017]{ACM Conference on Computer and Communications Security}{Due 19 May 2017}{Dallas, Texas}
\acmYear{2017}

% TODO: replace this section with code generated by the tool at https://dl.acm.org/ccs.cfm
\begin{CCSXML}
  <ccs2012>
  <concept>
  <concept_id>10002978.10002991.10002994</concept_id>concept_id>
  <concept_desc>Security and privacy~Pseudonymity, anonymity and untraceability</concept_desc>concept_desc>
  <concept_significance>500</concept_significance>concept_significance>
  </concept>concept>
  <concept>
  <concept_id>10002978.10002991.10002995</concept_id>concept_id>
  <concept_desc>Security and privacy~Privacy-preserving protocols</concept_desc>concept_desc>
  <concept_significance>500</concept_significance>concept_significance>
  </concept>concept>
  </ccs2012>ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy~Pseudonymity, anonymity and untraceability}
\ccsdesc[500]{Security and privacy~Privacy-preserving protocols}
% -- end of section to replace with generated code

\keywords{privacy, anonymity, messaging} % TODO: replace with your keywords


==> author-ieee.tex <==
%\author{\rm Paper \#50}
\author{
  \IEEEauthorblockN{Raymond Cheng\IEEEauthorrefmark{1}, xxx\IEEEauthorrefmark{2}}
  \IEEEauthorblockA{\IEEEauthorrefmark{1}UC Berkeley
  \\\{ryscheng, xxx\}@cs.berkeley.edu}
  \IEEEauthorblockA{\IEEEauthorrefmark{2}YYY
  \\yyy@uw.edu}
}


==> main.tex <==
\newif\ifOverleaf
\Overleaftrue
\input{paper-docclass}
\input{paper-common}


==> paper-docclass.tex <==
% style/head-* files has \documentclass but arxiv looks for it, so the
% entry points paper.tex for normal use, main.tex for overleaf, and
% arxiv.tex for arxiv's autotex to recognize and use need this
% separated out.

%\input{style/head-acm}
%\input{style/head-ieee}
%\input{style/head-usenix} % usenix style has no date
\input{style/head-plain}
%\input{style/head-plain-1col}


==> paper.tex <==
\newif\ifOverleaf
\Overleaffalse
\input{paper-docclass}
\input{paper-common}

